Strong Formulations for Hybrid System Control

We study the mixed-integer quadratic programming formulation of an $n$-period hybrid control problem with a convex quadratic cost function and linear dynamics. We first give the convex hull description of the single-period, two-mode problem in the original variable space through two new classes of valid cuts. These cuts are then generalized to the single-period, multi-mode, multi-dimensional case and applied to solve the general $n$-period hybrid control problem. Computational experiments demonstrate the effectiveness of the proposed strong formulations derived through the cut generation process in the original variable space. These formulations yield a substantial reduction in computational effort for synthetic test instances and instances from the energy management problem of a power-split hybrid electric vehicle.

==> tables/HEV_result_newDynamics_arXiv.tex <==
\begin{tabular}{p{0.15cm}|p{0.2cm}|p{0.2cm}|p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}}
\hline \hline
\multicolumn{3}{c|}{Sampling Time}  & \multicolumn{6}{c|}{$T_s=1$ sec} & \multicolumn{6}{c}{$T_s=0.5$ sec} \\ \hline
 \multicolumn{3}{c|}{Instance}  & \multicolumn{2}{c|}{Relax. Gap (\%)} & \multicolumn{2}{c|}{Comp. Time (sec)} & \multicolumn{2}{c|}{\# Branch}   & \multicolumn{2}{c|}{Relax. Gap (\%)} & \multicolumn{2}{c|}{Comp. Time (sec)} & \multicolumn{2}{c}{\# Branch}   \\ \hline
 \multicolumn{1}{c|}{$r_1$} & \multicolumn{1}{c|}{$\gamma$} & \multicolumn{1}{c|}{Metrics} & \multicolumn{1}{c}{MIQP}  & \multicolumn{1}{c|}{WC-G}   & \multicolumn{1}{c}{MIQP} & \multicolumn{1}{c|}{WC-G}   & \multicolumn{1}{c}{MIQP} & \multicolumn{1}{c|}{WC-G}   & \multicolumn{1}{c}{MIQP}  & \multicolumn{1}{c|}{WC-G}   & \multicolumn{1}{c}{MIQP} & \multicolumn{1}{c|}{WC-G}   & \multicolumn{1}{c}{MIQP} & \multicolumn{1}{c}{WC-G}   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{$1$}} & \multicolumn{1}{c|}{\multirow{2}{*}{$0$}} & \multicolumn{1}{c|}{Avg.}                                                                & \multicolumn{1}{c}{46.51}  & \multicolumn{1}{c|}{19.10} & \multicolumn{1}{c}{2.85}   & \multicolumn{1}{c|}{3.06}   & \multicolumn{1}{c}{2393.20}  &  \multicolumn{1}{c|}{826.76}  & \multicolumn{1}{c}{64.56}  & \multicolumn{1}{c|}{15.71} & \multicolumn{1}{c}{2.80}   & \multicolumn{1}{c|}{0.44}   & \multicolumn{1}{c}{2047.31}  &  \multicolumn{1}{c}{200.96}  \\ % \cline{3-15} 
& &\multicolumn{1}{c|}{Max}                                                                 & \multicolumn{1}{c}{99.17}  & \multicolumn{1}{c|}{96.46} & \multicolumn{1}{c}{57.95}  & \multicolumn{1}{c|}{122.58} & \multicolumn{1}{c}{45138}    & \multicolumn{1}{c|}{32447}   & \multicolumn{1}{c}{99.16}  & \multicolumn{1}{c|}{97.82} & \multicolumn{1}{c}{182.62} & \multicolumn{1}{c|}{7.91}   & \multicolumn{1}{c}{77682}    & \multicolumn{1}{c}{3981}    \\ \cline{2-15} 
 & \multicolumn{1}{c|}{\multirow{2}{*}{$0.01$}} & \multicolumn{1}{c|}{Avg.}                                                                & \multicolumn{1}{c}{43.79}  & \multicolumn{1}{c|}{20.96} & \multicolumn{1}{c}{2.49}   & \multicolumn{1}{c|}{2.37}   & \multicolumn{1}{c}{2812.38}  & \multicolumn{1}{c|}{602.04}  & \multicolumn{1}{c}{68.45}  & \multicolumn{1}{c|}{13.37} & \multicolumn{1}{c}{1.68}   & \multicolumn{1}{c|}{0.61}   & \multicolumn{1}{c}{1569.15}  &  \multicolumn{1}{c}{212.53}  \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}                                                       & \multicolumn{1}{c}{99.19}  & \multicolumn{1}{c|}{96.40} & \multicolumn{1}{c}{46.31}  & \multicolumn{1}{c|}{35.97}  & \multicolumn{1}{c}{38406}    &  \multicolumn{1}{c|}{8158}    & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{93.32} & \multicolumn{1}{c}{52.32}  & \multicolumn{1}{c|}{13.49}  & \multicolumn{1}{c}{18747}    &  \multicolumn{1}{c}{3307}    \\ \cline{2-15} 
& \multicolumn{1}{c|}{\multirow{2}{*}{$0.02$}} & \multicolumn{1}{c|}{Avg.}                                                                & \multicolumn{1}{c}{43.56}  & \multicolumn{1}{c|}{20.65} & \multicolumn{1}{c}{3.45}   & \multicolumn{1}{c|}{2.92}   & \multicolumn{1}{c}{3042.63}  &\multicolumn{1}{c|}{785.40}  & \multicolumn{1}{c}{72.60}  & \multicolumn{1}{c|}{16.31} & \multicolumn{1}{c}{4.04}   & \multicolumn{1}{c|}{0.51}   & \multicolumn{1}{c}{3060.89}  & \multicolumn{1}{c}{223.90}  \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}   & \multicolumn{1}{c}{99.06}  & \multicolumn{1}{c|}{98.54} & \multicolumn{1}{c}{65.55}  & \multicolumn{1}{c|}{36.56}  & \multicolumn{1}{c}{41989}    & \multicolumn{1}{c|}{10286}   & \multicolumn{1}{c}{98.88}  & \multicolumn{1}{c|}{91.41} & \multicolumn{1}{c}{192.57} & \multicolumn{1}{c|}{14.79}  & \multicolumn{1}{c}{76353}    & \multicolumn{1}{c}{4541}    \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{$10$}} & \multicolumn{1}{c|}{\multirow{2}{*}{$0$}} & \multicolumn{1}{c|}{Avg.}                                                                & \multicolumn{1}{c}{51.72}  & \multicolumn{1}{c|}{18.03} & \multicolumn{1}{c}{29.27}  & \multicolumn{1}{c|}{17.36}  & \multicolumn{1}{c}{13064.27} & \multicolumn{1}{c|}{2871.15} & \multicolumn{1}{c}{60.02}  & \multicolumn{1}{c|}{14.51} & \multicolumn{1}{c}{48.63}  & \multicolumn{1}{c|}{11.36}  & \multicolumn{1}{c}{25072.97} & \multicolumn{1}{c}{1977.94} \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}          & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{92.84} & \multicolumn{1}{c}{466.59} & \multicolumn{1}{c|}{315.72} & \multicolumn{1}{c}{120023}   & \multicolumn{1}{c|}{59936}   & \multicolumn{1}{c}{99.36}  & \multicolumn{1}{c|}{92.32} & \multicolumn{1}{c}{570.77} & \multicolumn{1}{c|}{303.09} & \multicolumn{1}{c}{179272}   & \multicolumn{1}{c}{50581}   \\ \cline{2-15} 
& \multicolumn{1}{c|}{\multirow{2}{*}{$0.01$}} & \multicolumn{1}{c|}{Avg.}                                                                & \multicolumn{1}{c}{45.50}  & \multicolumn{1}{c|}{19.77} & \multicolumn{1}{c}{35.69}  & \multicolumn{1}{c|}{14.85}  & \multicolumn{1}{c}{12101.21} & \multicolumn{1}{c|}{2419.21} & \multicolumn{1}{c}{61.95}  & \multicolumn{1}{c|}{18.11} & \multicolumn{1}{c}{30.44}  & \multicolumn{1}{c|}{10.10}  & \multicolumn{1}{c}{17260.90} & \multicolumn{1}{c}{1597.82} \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}  & \multicolumn{1}{c}{99.14}  & \multicolumn{1}{c|}{96.78} & \multicolumn{1}{c}{571.23} & \multicolumn{1}{c|}{505.43} & \multicolumn{1}{c}{142084}   & \multicolumn{1}{c|}{68744}   & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{95.85} & \multicolumn{1}{c}{567.99} & \multicolumn{1}{c|}{385.29} & \multicolumn{1}{c}{153765}   & \multicolumn{1}{c}{52270}   \\ \cline{2-15} 
 & \multicolumn{1}{c|}{\multirow{2}{*}{$0.02$}} & \multicolumn{1}{c|}{Avg.}  & \multicolumn{1}{c}{47.08}  & \multicolumn{1}{c|}{17.95} & \multicolumn{1}{c}{20.77}  & \multicolumn{1}{c|}{10.70}  & \multicolumn{1}{c}{12146.60} & \multicolumn{1}{c|}{1877.74} & \multicolumn{1}{c}{66.04}  & \multicolumn{1}{c|}{15.39} & \multicolumn{1}{c}{52.05}  & \multicolumn{1}{c|}{14.94}  & \multicolumn{1}{c}{24346.68} & \multicolumn{1}{c}{2467.67} \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}                                                                  & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{98.23} & \multicolumn{1}{c}{255.77} & \multicolumn{1}{c|}{327.40} & \multicolumn{1}{c}{123163}   & \multicolumn{1}{c|}{66240}   & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{97.43} & \multicolumn{1}{c}{518.10} & \multicolumn{1}{c|}{304.35} & \multicolumn{1}{c}{170175}   & \multicolumn{1}{c}{49313}   \\ \hline
\multicolumn{1}{c|}{\multirow{6}{*}{$100$}} & \multicolumn{1}{c|}{\multirow{2}{*}{$0$}} & \multicolumn{1}{c|}{Avg.} & \multicolumn{1}{c}{45.41}  & \multicolumn{1}{c|}{18.99} & \multicolumn{1}{c}{34.34}  & \multicolumn{1}{c|}{24.77}  & \multicolumn{1}{c}{11986.84} & \multicolumn{1}{c|}{3645.06} & \multicolumn{1}{c}{54.80}  & \multicolumn{1}{c|}{14.07} & \multicolumn{1}{c}{38.09}  & \multicolumn{1}{c|}{21.04}  & \multicolumn{1}{c}{22693.04} & \multicolumn{1}{c}{3483.76} \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max} & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{93.93} & \multicolumn{1}{c}{570.70} & \multicolumn{1}{c|}{413.64} & \multicolumn{1}{c}{116566}   & \multicolumn{1}{c|}{57238}   & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{97.47} & \multicolumn{1}{c}{590.54} & \multicolumn{1}{c|}{583.52} & \multicolumn{1}{c}{155165}   & \multicolumn{1}{c}{90511}   \\ \cline{2-15} 
 & \multicolumn{1}{c|}{\multirow{2}{*}{$0.01$}} & \multicolumn{1}{c|}{Avg.}  & \multicolumn{1}{c}{47.90}  & \multicolumn{1}{c|}{17.97} & \multicolumn{1}{c}{24.74}  & \multicolumn{1}{c|}{23.15}  & \multicolumn{1}{c}{11204.93} & \multicolumn{1}{c|}{3520.48} & \multicolumn{1}{c}{60.12}  & \multicolumn{1}{c|}{15.59} & \multicolumn{1}{c}{44.21}  & \multicolumn{1}{c|}{29.29}  & \multicolumn{1}{c}{26016.09} & \multicolumn{1}{c}{4425.76} \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}   & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{93.16} & \multicolumn{1}{c}{374.83} & \multicolumn{1}{c|}{318.33} & \multicolumn{1}{c}{125609}   & \multicolumn{1}{c|}{54807}   & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{89.71} & \multicolumn{1}{c}{599.90} & \multicolumn{1}{c|}{457.49} & \multicolumn{1}{c}{162050}   & \multicolumn{1}{c}{71808}   \\ \cline{2-15} 
 & \multicolumn{1}{c|}{\multirow{2}{*}{$0.02$}} & \multicolumn{1}{c|}{Avg.}& \multicolumn{1}{c}{41.45}  & \multicolumn{1}{c|}{26.87} & \multicolumn{1}{c}{35.24}  & \multicolumn{1}{c|}{19.10}  & \multicolumn{1}{c}{12958.20} & \multicolumn{1}{c|}{3031.26} & \multicolumn{1}{c}{63.59}  & \multicolumn{1}{c|}{16.33} & \multicolumn{1}{c}{53.19}  & \multicolumn{1}{c|}{28.65}  & \multicolumn{1}{c}{28578.54} & \multicolumn{1}{c}{4482.11} \\ % \cline{3-15} 
& & \multicolumn{1}{c|}{Max}                                                                  & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{93.99} & \multicolumn{1}{c}{540.72} & \multicolumn{1}{c|}{297.54} & \multicolumn{1}{c}{116676}   & \multicolumn{1}{c|}{43022}   & \multicolumn{1}{c}{100.00} & \multicolumn{1}{c|}{97.87} & \multicolumn{1}{c}{476.74} & \multicolumn{1}{c|}{432.31} & \multicolumn{1}{c}{158678}   & \multicolumn{1}{c}{81983}   \\ \hline 
\multicolumn{3}{c|}{\textbf{Overall Average}} & \multicolumn{1}{c}{\textbf{39.37}}  & \multicolumn{1}{c|}{\textbf{27.50}} & \multicolumn{1}{c}{\textbf{20.98}}  & \multicolumn{1}{c|}{\textbf{13.14}}  & \multicolumn{1}{c}{\textbf{9078.92}}  & \multicolumn{1}{c|}{\textbf{2175.46}} & \multicolumn{1}{c}{\textbf{63.57}}  & \multicolumn{1}{c|}{\textbf{15.49}} & \multicolumn{1}{c}{\textbf{30.57}}  & \multicolumn{1}{c|}{\textbf{12.99}}  & \multicolumn{1}{c}{\textbf{16738.40}} & \multicolumn{1}{c}{\textbf{2119.16}} \\ \hline \hline
\end{tabular}

